Ever: Mitigating Hallucination in Large Language Models through Real-Time Verification and Rectification

Large Language Models (LLMs) have demonstrated remarkable proficiency in generating fluent text. However, they often encounter the challenge of generating inaccurate or hallucinated content. This issue is common in both non-retrieval-based generation and retrieval-augmented generation approaches, and existing post-hoc rectification methods may not address the accumulated hallucination errors that may be caused by the "snowballing" issue, especially in reasoning tasks. To tackle these challenges, we introduce a novel approach called Real-time Verification and Rectification (Ever). Instead of waiting until the end of the generation process to rectify hallucinations, Ever employs a real-time, step-wise generation and hallucination rectification strategy. The primary objective is to detect and rectify hallucinations as they occur during the text generation process. When compared to both retrieval-based and non-retrieval-based baselines, Ever demonstrates a significant improvement in generating trustworthy and factually accurate text across a diverse range of tasks, including short-form QA, biography generation, and multi-hop reasoning.

==> trash.tex <==
To increase the factuality of LLMs:

1. Decoding \cite{chuang2023dola} \cite{shi2023trusting} \cite{li2022contrastive} \cite{li2023inference}
2. post-hoc attribution (retrieval)\cite{peng2023check} \cite{gao2022attributed} \cite{chern2023factool} \cite{yu2023improving} \cite{varshney2023stitch} (non-retrieval) \cite{dhuliawala2023chain} 
3. RAG: \cite{lewis2020retrieval}  \cite{jiang2023active} \cite{asai2023self}
4. training-time methods: Reinforcement learning \cite{roit2023factually}\cite{wu2023fine} Contrastive learning \cite{chern2023improving} \cite{sun2023contrastive}  other methods \cite{li2023inference}


\begin{table*}[ht]
    \centering
    \begin{tabular}{ccccc}
        \toprule
        \textsc{$\mathrm{LM}_{gen}$}  & \texttt{FactScore.(\%)} &  Avg. \# facts \\
        \toprule
        \multicolumn{3}{c}{\textit{Without Retrieval}} \\
        Llama 2 7B Chat  &36.8 & 23.5 \\
        Llama 2 13B Chat  &40.0 & 25.5 \\
        InstructGPT  &47.6 & 26.3\\
        GPT 3.5 Turbo   &65.1 & 34.7 \\
        Ours (Self-query)$_{7B}$& 46.7 &17.8 \\
         Ours (Self-query)$_{13B}$& 47.5 & 18.6 \\
         Ours (Self-query)$_{GPT3.5}$ & 73.2 & 20.4 \\

        \midrule

        \multicolumn{3}{c}{\textit{Post-Edit with Retrieval}} \\
        RRAR$_{7B}$ & 37.8 & 10.6 \\

        RRAR$_{13B}$ & 41.5 & 10.6 \\
        RRAR$_{GPT3.5}$& 74.3 & 19.2 \\
        
        Ours (Edit Only)$_{7B}$ & 76.9 & 20.1 \\
        Ours (Edit Only)$_{13B}$ & 78.5 & 21.1 \\
        Ours (Edit Only)$_{GPT3.5}$ & \textbf{94.5} & 39.2 \\

        \midrule

        \multicolumn{3}{c}{\textit{Retrieval then Generation}} \\
        PerplexityAI  & 72.3 & 40.8 \\
        RAG$_{7B}$ &  78.0 & - \\  
        Self-RAG$_{7B}$ & 81.2  & - \\ 
        
        RAG$_{13B}$ & 77.5 & - \\  
        Self-RAG$_{13B}$ & 80.2  & - \\ 
         Ours (Retr + Edit)$_{7B}$ & 88.3 & 20.7 \\
         Ours (Retr + Edit)$_{13B}$ & 89.6 & 20.9 \\
         Ours (Retr + Edit)$_{GPT3.5}$ & \textbf{95.8} & 40.5 \\

        \midrule

         Ours (Self-query)$_{7B}$& 46.7 &17.8 \\
        Ours (Edit Only)$_{7B}$ & 76.9 & 20.1 \\
         Ours (Retr + Edit)$_{7B}$ & 88.3 & 20.7 \\

         Ours (Self-query)$_{13B}$& 47.5 & 18.6 \\
         Ours (Edit Only)$_{13B}$ & 79.5 & 21.1 \\
         Ours (Retr + Edit)$_{13B}$ & 89.6 & 20.9 \\
    
         Ours (Self-query)$_{GPT3.5}$ & 73.2 & 20.4 \\
        Ours (Edit Only)$_{GPT3.5}$ & \textbf{94.5} & 39.2 \\
         Ours (Retr + Edit)$_{GPT3.5}$ & \textbf{95.8} & 40.5 \\

        \bottomrule
    \end{tabular}
    \caption{Results on the biography generation task. }
    \label{tab:bio_main}
\end{table*}


\begin{table}[ht]
    \caption{Results on the biography generation task. $^*$These numbers are from \citet{asai2023self}. $^\dagger$We obtain the results from \citet{dhuliawala2023chain}.}
    \vspace{-0.5em}
    \centering
    \small
    \resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{1mm}{
    \begin{tabular}{lcc}
        \toprule
        LM Scale & Method & \textsc{FactScore} (\%)  \\
        \toprule
        \multicolumn{3}{c}{\textit{Non-Retrieval}} \vspace{0.3em}\\
        InstructGPT  & Zero-Shot &47.6 \\
        
        \noalign{\smallskip} \hdashline \noalign{\smallskip}
        %\noalgin \vspace{0.01em} \hdashline \vspace{0.01em}

        \multirow{3}{*}{Llama 2 7B Chat} & Zero-Shot &36.8 \\
                                        & Dola &36.8 \\
                                        &\textsc{Ever (nrg+sq)}& 46.7 \\
        
        \noalign{\smallskip} \hdashline \noalign{\smallskip}
        \multirow{3}{*}{Llama 2 13B Chat} & Zero-Shot &40.3 \\
                                        & Dola &40.1 \\
                                        &\textsc{Ever (nrg+sq)}& 47.5 \\
                                        
        \noalign{\smallskip} \hdashline \noalign{\smallskip}
        \multirow{3}{*}{Llama 1 65B} & Few-Shot$^\dagger$ & 55.9 \\
                                         & CoVe$^\dagger$ & 71.4  \\
                                        & \textsc{Ever (nrg+sq)} &72.9 \\
                                        
        \noalign{\smallskip} \hdashline \noalign{\smallskip}
        \multirow{2}{*}{GPT 3.5 Tubro} & Zero-Shot &71.8 \\
                                        &\textsc{Ever (nrg+sq)}& \textbf{75.2} \\
                                        
        %Llama 2 7B Chat  &36.8  \\
        %Llama 2 13B Chat  &40.0  \\
        
        %Dola$_{7B}$ & 41.4 \\ 
        %Dola$_{13B}$ & 40.1  \\ 
        %\textsc{Ever (nrg+sq)}$_{7B}$& 46.7  \\
         %\textsc{Ever (nrg+sq)}$_{13B}$& 47.5  \\
         %\textsc{Ever (nrg+sq)}$_{\rm{GPT}3.5}$ & \textsc{Ever (nrg+sq)} & \textbf{73.2}  \\

        \midrule

        \multicolumn{3}{c}{\textit{Retrieval-Augmented Rectification}} \vspace{0.3em}\\
        
        \multirow{2}{*}{Llama 2 7B Chat} & RRAR &37.8  \\
                                        & \textsc{Ever (nrg+er)} &76.9 \\        
        \noalign{\smallskip} \hdashline \noalign{\smallskip}

        \multirow{2}{*}{Llama 2 13B Chat} & RRAR &41.5  \\
                                        & \textsc{Ever (nrg+er)} &79.5 \\        
        \noalign{\smallskip} \hdashline \noalign{\smallskip}
        \multirow{2}{*}{GPT 3.5 Turbo} & RRAR & 74.3 \\
                                        & \textsc{Ever (nrg+er)} &\textbf{94.5} \\        
        \midrule

        \multicolumn{3}{c}{\textit{Retrieval-Augmented Generation and Rectification}} \vspace{0.3em}\\
        PerplexityAI  & RAG & 40.8 \\ 
        \noalign{\smallskip} \hdashline \noalign{\smallskip}
        \multirow{3}{*}{Llama 2 7B Chat} & RAG &79.4  \\
                                        & Self-RAG$^*$ & 81.2 \\
                                        & \textsc{Ever (rag+er)} & 86.4 \\        
        \noalign{\smallskip} \hdashline \noalign{\smallskip}
        
        \multirow{3}{*}{Llama 2 13B Chat} & RAG$^*$ & 79.9  \\
                                        & Self-RAG$^*$ & 80.2 \\
                                        & \textsc{Ever (rag+er)} & 87.3 \\        
        \noalign{\smallskip} \hdashline \noalign{\smallskip}
        
        \multirow{2}{*}{GPT 3.5 Turbo} & RAG & 92.7  \\
                                    & \textsc{Ever (rag+er)} & \textbf{95.8}\\        
        \bottomrule
    \end{tabular}}}
    \label{tab:bio_main}
\end{table}


\begin{table}[ht]
    \caption{Results on the biography generation task. $^*$These numbers are from \citet{asai2023self}.}
    \vspace{-0.5em}
    \centering
    \small
    \resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{1mm}{
    \begin{tabular}{lcc}
        \toprule
        LM  & Method & FactScore (\%)  \\
        \toprule
        \multicolumn{3}{c}{\textit{Non-Retrieval}} \vspace{0.3em}\\
        Llama 2 7B Chat  &36.8 & 23.5 \\
        Llama 2 13B Chat  &40.0 & 25.5 \\
        InstructGPT  &47.6 & 26.3\\
        GPT 3.5 Turbo   &65.1 & 34.7 \\
        CoVe (Llama-65B) & 71.4 & 12.3 \\
        Dola$_{7B}$ & 41.4 &24.7 \\ 
        Dola$_{13B}$ & 40.1 & 27.2 \\ 
        IVM (NRG+SQ)$_{7B}$& 46.7 &17.8 \\
         IVM (NRG+SQ)$_{13B}$& 47.5 & 18.6 \\
         IVM (NRG+SQ)$_{\rm{GPT}3.5}$ & \textbf{73.2} & 20.4 \\

        \midrule

        \multicolumn{3}{c}{\textit{Retrieval-Augmented Rectification}} \vspace{0.3em}\\
        RRAR$_{7B}$ & 37.8 & 10.6 \\

        RRAR$_{13B}$ & 41.5 & 10.6 \\
        RRAR$_{\rm{GPT}3.5}$& 74.3 & 19.2 \\
        
        IVM (NRG+ER)$_{7B}$ & 76.9 & 20.1 \\
        IVM (NRG+ER)$_{13B}$ & 79.5 & 21.1 \\
        IVM (NRG+ER)$_{\rm{GPT}3.5}$ & \textbf{94.5} & 39.2 \\

        \midrule

        \multicolumn{3}{c}{\textit{Retrieval-Augmented Generation and Rectification}} \vspace{0.3em}\\
        PerplexityAI  & 72.3 & 40.8 \\
        $^*$RAG$_{7B}$ &  78.0 & - \\  
        $^*$Self-RAG$_{7B}$ & 81.2  & - \\ 
        
        $^*$RAG$_{13B}$ & 77.5 & - \\  
        $^*$Self-RAG$_{13B}$ & 80.2  & - \\ 
         IVM (RAG+ER)$_{7B}$ & 86.4 & 20.7 \\
         IVM (RAG+ER)$_{13B}$ & 87.3 & 20.9 \\
         IVM (RAG+ER)$_{\rm{GPT}3.5}$ & \textbf{95.8} & 40.5 \\

        \bottomrule
    \end{tabular}}}
    \label{tab:bio_main}
\end{table}
